Punctuation Matters! Stealthy Backdoor Attack for Language Models

Recent studies have pointed out that natural language processing (NLP) models are vulnerable to backdoor attacks. A backdoored model produces normal outputs on the clean samples while performing improperly on the texts with triggers that the adversary injects. However, previous studies on textual backdoor attack pay little attention to stealthiness. Moreover, some attack methods even cause grammatical issues or change the semantic meaning of the original texts. Therefore, they can easily be detected by humans or defense systems. In this paper, we propose a novel stealthy backdoor attack method against textual models, which is called \textbf{PuncAttack}. It leverages combinations of punctuation marks as the trigger and chooses proper locations strategically to replace them. Through extensive experiments, we demonstrate that the proposed method can effectively compromise multiple models in various tasks. Meanwhile, we conduct automatic evaluation and human inspection, which indicate the proposed method possesses good performance of stealthiness without bringing grammatical issues and altering the meaning of sentences.

==> ref.tex <==
%\bibitem{ref_article1}
% Author, F.: Article title. Journal \textbf{2}(5), 99--110 (2016)

% \bibitem{ref_lncs1}
% Author, F., Author, S.: Title of a proceedings paper. In: Editor,
% F., Editor, S. (eds.) CONFERENCE 2016, LNCS, vol. 9999, pp. 1--13.
% Springer, Heidelberg (2016). \doi{10.10007/1234567890}

% \bibitem{ref_book1}
% Author, F., Author, S., Author, T.: Book title. 2nd edn. Publisher,
% Location (1999)

% \bibitem{ref_proc1}
% Author, A.-B.: Contribution title. In: 9th International Proceedings
% on Proceedings, pp. 1--2. Publisher, Location (2010)

% \bibitem{ref_url1}
% LNCS Homepage, \url{http://www.springer.com/lncs}. Last accessed 4
% Oct 2017

% \bibitem{lecun2015deep}
% %author = {LeCun, Yann and Bengio, Yoshua and Hinton, Geoffrey},
% Y. LeCun, Y. Bengio, and G. Hinton: Deep learning. Nature(2015)
bibitem{lecun2015deep}
  title={Deep learning},
  author={LeCun, Yann and Bengio, Yoshua and Hinton, Geoffrey},
  journal={Nature},
  year={2015},
  url={https://doi.org/10.1038/nature14539}


\bibitem{bert}
J. D. M.-W. C. Kenton and L. K. Toutan
 author = {Jacob Devlin and
Ming{-}Wei Chang and
Kenton Lee and
Kristina Toutanova},
 booktitle = {Proc. of AACL},
 title = {{BERT:} Pre-training of Deep Bidirectional Transformers for Language Understanding},
 year = {2019}

\bibitem{gpt3}
 author = {Tom B. Brown and
Benjamin Mann and
Nick Ryder and
Melanie Subbiah and
Jared Kaplan and
Prafulla Dhariwal and
Arvind Neelakantan and
Pranav Shyam and
Girish Sastry and
Amanda Askell and
Sandhini Agarwal and
Ariel Herbert{-}Voss and
Gretchen Krueger and
Tom Henighan and
Rewon Child and
Aditya Ramesh and
Daniel M. Ziegler and
Jeffrey Wu and
Clemens Winter and
Christopher Hesse and
Mark Chen and
Eric Sigler and
Mateusz Litwin and
Scott Gray and
Benjamin Chess and
Jack Clark and
Christopher Berner and
Sam McCandlish and
Alec Radford and
Ilya Sutskever and
Dario Amodei},
 booktitle = {NeurIPS},
 title = {Language Models are Few-Shot Learners},
 year = {2020}

\bibitem{adversarial_survery}
 author = {Zhang, Wei Emma and Sheng, Quan Z and Alhazmi, Ahoud and Li, Chenliang},
 journal = {TIST},
 title = {Adversarial attacks on deep-learning models in natural language processing: A survey},
 year = {2020}

\bibitem{extract_data}
 author = {Nicholas Carlini and
Florian Tram{\`{e}}r and
Eric Wallace and
Matthew Jagielski and
Ariel Herbert{-}Voss and
Katherine Lee and
Adam Roberts and
Tom B. Brown and
Dawn Song and
{\'{U}}lfar Erlingsson and
Alina Oprea and
Colin Raffel},
 booktitle = {USENIX},
 title = {Extracting training data from large language models},
 year = {2021}

\bibitem{extract_model}
 author = {He, Xuanli and Lyu, Lingjuan and Sun, Lichao and Xu, Qiongkai},
 booktitle = {Proc. of AACL},
 title = {Model Extraction and Adversarial Transferability, Your BERT is Vulnerable!},
 year = {2021}

\bibitem{backdoorssurvey}
 author = {Li, Yiming and Wu, Baoyuan and Jiang, Yong and Li, Zhifeng and Xia, Shu-Tao},
 journal = {arXiv preprint arXiv:2007.08745},
 title = {Backdoor learning: A survey},
 year = {2020}

\bibitem{bd_translation}
 author = {Wallace, Eric and Zhao, Tony and Feng, Shi and Singh, Sameer},
 booktitle = {Proc. of AACL},
 title = {Concealed Data Poisoning Attacks on NLP Models},
 year = {2021}

\bibitem{ccs_shen}
 author = {Lujia Shen and
Shouling Ji and
Xuhong Zhang and
Jinfeng Li and
Jing Chen and
Jie Shi and
Chengfang Fang and
Jianwei Yin and
Ting Wang},
 booktitle = {CCS},
 title = {Backdoor Pre-trained Models Can Transfer to All},
 year = {2021}

\bibitem{ripples}
 author = { Kurita, K.  and  Michel, P.  and  Neubig, G. },
 booktitle = {ACL},
 title = {Weight Poisoning Attacks on Pre-trained Models},
 year = {2020}

\bibitem{textstyle}
 author = {Fanchao Qi and
Yangyi Chen and
Xurui Zhang and
Mukai Li and
Zhiyuan Liu and
Maosong Sun},
 booktitle = {EMNLP},
 title = {Mind the Style of Text! Adversarial and Backdoor Attacks Based on Text Style Transfer},
 year = {2021}

\bibitem{subs}
 author = {Fanchao Qi and
Yuan Yao and
Sophia Xu and
Zhiyuan Liu and
Maosong Sun},
 booktitle = {ACL/IJCNLP},
 title = {Turn the Combination Lock: Learnable Textual Backdoor Attacks via Word Substitution},
 year = {2021}

\bibitem{stealthiness}
 author = {Yang, Wenkai and Lin, Yankai and Li, Peng and Zhou, Jie and Sun, Xu},
 booktitle = {ACL/IJCNLP},
 title = {Rethinking Stealthiness of Backdoor Attack against NLP Models},
 year = {2021}

\bibitem{insertsent}
 author = {Dai, Jiazhu and Chen, Chuanshuai and Li, Yufeng},
 journal = {IEEE Access},
 title = {A backdoor attack against lstm-based text classification systems},
 year = {2019}

\bibitem{hiddenkiller}
author = {Fanchao Qi and
Mukai Li and
Yangyi Chen and
Zhengyan Zhang and
Zhiyuan Liu and
Yasheng Wang and
Maosong Sun},
 booktitle = {ACL/IJCNLP},
 title = {Hidden Killer: Invisible Textual Backdoor Attacks with Syntactic Trigger},
 year = {2021}

\bibitem{tminer}
 author = {Azizi, Ahmadreza and Tahmid, Ibrahim Asadullah and Waheed, Asim and Mangaokar, Neal and Pu, Jiameng and Javed, Mobin and Reddy, Chandan K and Viswanath, Bimal},
 booktitle = {USENIX},
 title = {T-Miner: A Generative Approach to Defend Against Trojan Attacks on DNN-based Text Classification},
 year = {2021}

\bibitem{commas}
 author = {Hill, Robin L and Murray, Wayne S},
 journal = {11th Annual CUNY Con ference on Human Sentence Processing.},
 title = {Commas and spaces: The point of punctuation},
 year = {1998}

\bibitem{visible}
 author = {Toner, Anne},
 journal = {Visible Language},
 title = {Seeing punctuation},
 year = {2011}

\bibitem{ripples_free}
 author = {Yang, Wenkai and Li, Lei and Zhang, Zhiyuan and Ren, Xuancheng and Sun, Xu and He, Bin},
 booktitle = {Proc. of AACL},
 title = {Be Careful about Poisoned Word Embeddings: Exploring the Vulnerability of the Embedding Layers in NLP Models},
 year = {2021}

\bibitem{layerwise}
 author = {Linyang Li and
Demin Song and
Xiaonan Li and
Jiehang Zeng and
Ruotian Ma and
Xipeng Qiu},
 booktitle = {EMNLP},
 title = {Backdoor Attacks on Pre-trained Models by Layerwise Weight Poisoning},
 year = {2021}

\bibitem{red}
 author = {Zhang, Zhengyan and Xiao, Guangxuan and Li, Yongwei and Lv, Tian and Qi, Fanchao and  et al.},
 journal = {MIR},
 title = {Red Alarm for Pre-trained Models: Universal Vulnerability to Neuron-Level Backdoor Attacks},
 year = {2021}

\bibitem{qa_ccs}
 author = {Shaofeng Li and
Hui Liu and
Tian Dong and
Benjamin Zi Hao Zhao and
Minhui Xue and
Haojin Zhu and
Jialiang Lu},
 booktitle = {CCS},
 title = {Hidden Backdoors in Human-Centric Language Models},
 year = {2021}

\bibitem{qa1}
 author = {Zhang, Xinyang and Zhang, Zheng and Ji, Shouling and Wang, Ting},
 booktitle = {EuroSandP},
 title = {Trojaning language models for fun and profit},
 year = {2021}

\bibitem{ag}
 author = {Xiang Zhang and
Junbo Jake Zhao and
Yann LeCun},
 booktitle = {NeurIPS},
 title = {Character-level Convolutional Networks for Text Classification},
 year = {2015}

\bibitem{imdb}
 author = {Andrew L. Maas and
Raymond E. Daly and
Peter T. Pham and
Dan Huang and
Andrew Y. Ng and
Christopher Potts},
 booktitle = {ACL},
 title = {Learning Word Vectors for Sentiment Analysis},
 year = {2011}

\bibitem{badnets}
 author = {Gu, Tianyu and Dolan-Gavitt, Brendan and Garg, Siddharth},
 journal = {arXiv preprint arXiv:1708.06733},
 title = {Badnets: Identifying vulnerabilities in the machine learning model supply chain},
 year = {2017}

\bibitem{bertscore}
 author = {Tianyi Zhang and
Varsha Kishore and
Felix Wu and
Kilian Q. Weinberger and
Yoav Artzi},
 booktitle = {ICLR},
 title = {BERTScore: Evaluating Text Generation with {BERT}},
 year = {2020}

\bibitem{squad}
 author = {Pranav Rajpurkar and
Jian Zhang and
Konstantin Lopyrev and
Percy Liang},
 booktitle = {EMNLP},
 title = {SQuAD: 100, 000+ Questions for Machine Comprehension of Text},
 year = {2016}



% \bibitem{transformer}
%  author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
%  booktitle = {NeurIPS},
%  title = {Attention is all you need},
%  year = {2017}

% \bibitem{gpt2}
%  author = {Radford, Alec and Wu, Jeffrey and Child, Rewon and Luan, David and Amodei, Dario and Sutskever, Ilya},
%  journal = {OpenAI blog},
%  title = {Language models are unsupervised multitask learners},
%  year = {2019}

% \bibitem{roberta}
%  author = {Liu, Yinhan and Ott, Myle and Goyal, Naman and Du, Jingfei and Joshi, Mandar and Chen, Danqi and Levy, Omer and Lewis, Mike and Zettlemoyer, Luke and Stoyanov, Veselin},
%  journal = {arXiv preprint arXiv:1907.11692},
%  title = {Roberta: A robustly optimized bert pretraining approach},
%  year = {2019}
